Rethinking Neural Nonlinearity as Gating

Activation functions are considered an essential primitive for neural nonlinearity, i.e., they enable neural networks to serve as universal approximators. In this paper, we show that this nonlinearity can also be achieved by input-conditioned threshold gating through branches as a universal primitive. We demonstrate that standard activations -- whether piecewise-linear (ReLU, PReLU, Hardtanh) or smooth (SiLU, Sigmoid, Tanh, GELU) -- are in fact instances of a single Threshold Gating (TG) primitive. For softmax, we show that it admits an exact TG conversion via its equivalent per-element Sigmoid form. We then validate these equivalences by converting pretrained networks across CNNs, transformer-based models, and recurrent architectures, preserving model performance without requiring retraining. Threshold Gating also enables training from scratch that goes beyond replacing existing activations, enabling gains in model compression, performance, and shorter training. We also propose a 'Minimal Branch Theorem' which relates the minimum number of required branches in our primitive to the trainability of general deep neural networks. In terms of hardware implementation, TG maps to a unified implementation in the case of analog in-memory systems, addressing the bottleneck of analog-to-digital and digital-to-analog converters (ADC/DAC) that is known to significantly impact power consumption and on-chip area.

==> figures/dissertation_colors.tex <==
% ============================================================================
% DISSERTATION COLOR SCHEME - CENTRAL CONTROL
% ============================================================================
% Change the 7 primary colors below to instantly update ALL figures.
% ============================================================================

% ----------------------------------------------------------------------------
% PRIMARY PALETTE - Wong 2011 Colorblind-Friendly (Nature Methods)
% ----------------------------------------------------------------------------
\definecolor{DissColor1}{HTML}{0072B2}   % Blue
\definecolor{DissColor2}{HTML}{E69F00}   % Orange
\definecolor{DissColor3}{HTML}{009E73}   % Bluish Green
\definecolor{DissColor4}{HTML}{CC79A7}   % Reddish Purple
\definecolor{DissColor5}{HTML}{8B0000}   % Dark Red (panel-c TG-LSTM, distinct from blue baseline)
\definecolor{DissColor6}{HTML}{D55E00}   % Vermillion
\definecolor{DissColor7}{HTML}{F0E442}   % Yellow

% ----------------------------------------------------------------------------
% dusty commented: Previous Dusty Muted Palette
% ----------------------------------------------------------------------------
% \definecolor{DissColor1}{HTML}{7080A8}   % Dusty Blue
% \definecolor{DissColor2}{HTML}{C97B72}   % Dusty Rose
% \definecolor{DissColor3}{HTML}{C8B070}   % Dusty Gold
% \definecolor{DissColor4}{HTML}{9966AA}   % Mauve
% \definecolor{DissColor5}{HTML}{88A878}   % Sage Mist
% \definecolor{DissColor6}{HTML}{80A8A8}   % Hazy Teal
% \definecolor{DissColor7}{HTML}{C07850}   % Burnt Sienna

% ----------------------------------------------------------------------------
% GRAYS
% ----------------------------------------------------------------------------
\definecolor{DissGray1}{RGB}{204,204,204}  % Grid gray (light)
\definecolor{DissGray2}{RGB}{176,176,176}  % Medium-light gray
\definecolor{DissGray3}{RGB}{128,128,128}  % Medium gray
\definecolor{DissGray4}{RGB}{244,244,244}  % Very light gray (background)

% ----------------------------------------------------------------------------
% FILL BLENDS (colour!N mixed with white) — for TikZ fill backgrounds
% ----------------------------------------------------------------------------
\colorlet{DissColor1Fill}{DissColor1!25}
\colorlet{DissColor2Fill}{DissColor2!30}
\colorlet{DissColor3Fill}{DissColor3!30}
\colorlet{DissColor4Fill}{DissColor4!30}
\colorlet{DissColor5Fill}{DissColor5!30}
\colorlet{DissColor6Fill}{DissColor6!25}
\colorlet{DissColor7Fill}{DissColor7!55}
\colorlet{DissColorIO}{black!10}

% ----------------------------------------------------------------------------
% TIKZPLOTLIB COMPATIBILITY (auto-generated figures use color0, color1, etc.)
% ----------------------------------------------------------------------------
\colorlet{color0}{DissColor1}
\colorlet{color1}{DissColor2}
\colorlet{color2}{DissColor3}
\colorlet{color3}{DissColor4}
\colorlet{color4}{DissColor5}
\colorlet{color5}{DissColor6}
\colorlet{color6}{DissColor7}

% Gray aliases for tikzplotlib
\colorlet{darkgray176}{DissGray2}
\colorlet{lightgray204}{DissGray1}
\colorlet{whitesmoke244}{DissGray4}
\colorlet{darkgray}{DissGray2}
\colorlet{lightgray}{DissGray1}

% ============================================================================
% CUSTOM HALF-FILLED MARKERS (for B&W scatter plot distinction)
% ============================================================================
% Half-filled circle (left half filled)
\pgfdeclareplotmark{halfcircle}{%
  \pgfpathcircle{\pgfpointorigin}{\pgfplotmarksize}
  \pgfusepath{stroke}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpatharc{90}{270}{\pgfplotmarksize}
  \pgfpathclose
  \pgfusepath{fill}
}

% Half-filled square (left half filled)
\pgfdeclareplotmark{halfsquare}{%
  \pgfpathrectangle
    {\pgfpoint{-\pgfplotmarksize}{-\pgfplotmarksize}}
    {\pgfpoint{2\pgfplotmarksize}{2\pgfplotmarksize}}
  \pgfusepath{stroke}
  \pgfpathrectangle
    {\pgfpoint{-\pgfplotmarksize}{-\pgfplotmarksize}}
    {\pgfpoint{\pgfplotmarksize}{2\pgfplotmarksize}}
  \pgfusepath{fill}
}

% ============================================================================
% CYCLE LISTS - Edit here to change ALL plots!
% ============================================================================

% ----------------------------------------------------------------------------
% BAR PATTERNS (for B&W printing compatibility)
% ----------------------------------------------------------------------------
% Requires: \usetikzlibrary{patterns}
\pgfplotscreateplotcyclelist{dissertation barplot patterns}{
  {fill=DissColor1, draw=black},
  {fill=DissColor2, draw=black, postaction={pattern=north east lines, pattern color=white}},
  {fill=DissColor3, draw=black, postaction={pattern=dots, pattern color=black!40}},
  {fill=DissColor4, draw=black, postaction={pattern=crosshatch, pattern color=white}},
  {fill=DissColor5, draw=black, postaction={pattern=horizontal lines, pattern color=white}},
  {fill=DissColor6, draw=black, postaction={pattern=north west lines, pattern color=black!40}},
  {fill=DissColor7, draw=black, postaction={pattern=grid, pattern color=white}},
}

% ----------------------------------------------------------------------------
% LINE PLOTS (with distinct markers & dashes)
% ----------------------------------------------------------------------------
\pgfplotscreateplotcyclelist{dissertation lineplot}{
  {line width=1.2pt, solid, color=DissColor1, mark=*, mark size=2.5, mark options={solid,draw=white}},
  {line width=1.2pt, solid, color=DissColor2, mark=square*, mark size=2.5, mark options={solid,draw=white}},
  {line width=1.2pt, solid, color=DissColor3, mark=triangle*, mark size=3, mark options={solid,draw=white}},
  {line width=1.2pt, solid, color=DissColor4, mark=diamond*, mark size=3, mark options={solid,draw=white}},
  {line width=1.2pt, solid, color=DissColor5, mark=pentagon*, mark size=3, mark options={solid,draw=white}},
  {line width=1.2pt, dashed, color=DissColor1, mark=o, mark size=2.5, mark options={solid}},
  {line width=1.2pt, dashed, color=DissColor2, mark=square, mark size=2.5, mark options={solid}},
  {line width=1.2pt, dotted, color=DissColor3, mark=triangle, mark size=3, mark options={solid}},
}

% ----------------------------------------------------------------------------
% SCATTER PLOTS (markers only, no lines)
% ----------------------------------------------------------------------------
\pgfplotscreateplotcyclelist{dissertation scatter}{
  {only marks, color=DissColor1, mark=*, mark size=3},
  {only marks, color=DissColor2, mark=square*, mark size=3},
  {only marks, color=DissColor3, mark=triangle*, mark size=3.5},
  {only marks, color=DissColor4, mark=diamond*, mark size=3.5},
  {only marks, color=DissColor5, mark=pentagon*, mark size=3},
  {only marks, color=DissColor6, mark=o, mark size=3},
  {only marks, color=DissColor7, mark=x, mark size=3.5},
}

% ============================================================================
% END - Change colors above to affect ALL plots!
% ============================================================================

